Sequential Ensembling for Semantic Segmentation

Ensemble approaches for deep-learning-based semantic segmentation remain insufficiently explored despite the proliferation of competitive benchmarks and downstream applications. In this work, we explore and benchmark the popular ensembling approach of combining predictions of multiple, independently-trained, state-of-the-art models at test time on popular datasets. Furthermore, we propose a novel method inspired by boosting to sequentially ensemble networks that significantly outperforms the naive ensemble baseline. Our approach trains a cascade of models conditioned on class probabilities predicted by the previous model as an additional input. A key benefit of this approach is that it allows for dynamic computation offloading, which helps deploy models on mobile devices. Our proposed novel ADaptive modulatiON (ADON) block allows spatial feature modulation at various layers using previous-stage probabilities. Our approach does not require sophisticated sample selection strategies during training and works with multiple neural architectures. We significantly improve over the naive ensemble baseline on challenging datasets such as Cityscapes, ADE-20K, COCO-Stuff, and PASCAL-Context and set a new state-of-the-art.

==> qualitative.tex <==
\begin{figure*}
\centering
\includegraphics[width=1\linewidth, height=0.4\linewidth]{images/3_experiments/qualitative/cityscapes/01.pdf}
\includegraphics[width=1\linewidth, height=0.4\linewidth]{images/3_experiments/qualitative/ade20k/01.pdf}
\includegraphics[width=1\linewidth, height=0.4\linewidth]{images/3_experiments/qualitative/ade20k/04.pdf}
\caption{Qualitative comparison of Sequential Ensembles and Simple Ensembles. Cityscapes (first three rows) and  ADE20K (last six rows) for HRNet-W48(N=2). The white eclipses highlight the fine-grained details that our approach captures in comparison to the baseline.}
\label{fig:qualitative}
\end{figure*}



==> tables/ade_coco_pascal.tex <==
\begin{table}[h]
    \centering
    \small
    
    %%% Notes on experiments, please don't delete.
    %%% ADE20k-deeplabv3+ are trained for 80k iterations (similar to cityscapes)
    %%% HRNets are trained for 160k iterations
    %%% mobilenetv3 are trained for 320k iterations. All details from mmsegmentation, we use LRASPP method (not FCN)
    %%% deeplabv3+ is better than PSPNet
    
    \resizebox{3.5in}{!}{
        \renewcommand{\arraystretch}{1.2} % Default value: 1, controls row space
        \begin{tabular}{@{}l|l | l | l | l@{}}
        \Xhline{3\arrayrulewidth}
           \textbf{Method} & \textbf{Arch} & \footnotesize{\textbf{ADE-20K}}  & \footnotesize{\textbf{COCO-Stuff}} & \footnotesize{\textbf{PASCAL-Context}}  \\
           \hline
           \footnotesize{MobileNetv3}~\cite{howard2019searching}  & D8s & 29.7 & 24.1 & 32.7 \\
           SIM-ENS & D8s & 31.4 (+1.7) & 26.3 (+2.2) & 34.2 (+1.5) \\
           SEQ-ENS & D8s & \textbf{35.3 (+5.6)} & \textbf{28.6 (+4.5)}  & \textbf{36.9 (+4.2)}\\
           
           \hline
           
           \footnotesize{MobileNetv3}~\cite{howard2019searching}  & D8 & 31.8 & 26.8 & 34.4 \\
           SIM-ENS & D8 & 33.9 (+2.1) & 28.5 (+1.7) & 36.0 (+1.6)\\
           SEQ-ENS & D8 & \textbf{35.6 (+3.8)} & \textbf{30.0 (+3.2)} & \textbf{37.3 (+2.9)}\\
            
            \hline \hline
            
            HRNet~\cite{sun2019high} & H-18s & 33.1 & 29.4 & 38.9 \\
            SIM-ENS & H-18s & 34.5 (+1.4) & 30.0 (+0.6) & 40.4 (+1.5) \\
            SEQ-ENS & H-18s & \textbf{37.6 (+4.5)} & \textbf{32.7 (+3.3)} & \textbf{42.0 (+3.1)} \\
            \hline
            
            HRNet~\cite{sun2019high} & H-18 & 36.8 & 33.0 & 42.6 \\
            SIM-ENS & H-18 & 37.6 (+0.8) & 34.1 (+1.1) & 43.9 (+1.3)\\
            SEQ-ENS & H-18 & \textbf{40.9 (+4.1)} & \textbf{35.7 (+2.7)} & \textbf{46.1 (+3.5)}\\
            \hline
            
            HRNet~\cite{sun2019high} & H-48 & 42.0 & 38.3 & 51.1\\
            SIM-ENS & H-48 & 42.5 (+0.5) & 39.7 (+1.4) & 52.1 (+1.0)\\
            SEQ-ENS & H-48 & \textbf{45.6 (+3.6)} & \textbf{40.8 (+2.5)} & \textbf{53.8 (+2.7)} \\
            \hline \hline
            
            DeepLabv3+~\cite{chen2018encoder} & R-18 & 34.1 & 29.7 & 43.5 \\
            SIM-ENS & R-18 & 35.4 (+1.3) & 31.2 (+1.5) & 45.8 (+2.3)  \\
            SEQ-ENS & R-18 & \textbf{37.6 (+3.5)} & \textbf{35.3 (+4.1)} & \textbf{46.2 (+2.7)}\\
            \hline
            
            DeepLabv3+~\cite{chen2018encoder} & R-50 & 42.7 & 37.4 & 50.4 \\
            SIM-ENS & R-50 & 43.3 (+0.6) & 38.2 (+0.8) & 51.8 (+1.4)\\
            SEQ-ENS & R-50 & \textbf{45.1 (+2.4)} & \textbf{39.2 (+1.8)} &  \textbf{52.4 (+2.0)}\\
            \hline
            
            DeepLabv3+~\cite{chen2018encoder} & R-101 & 44.6 & 38.8 & 53.2\\
            SIM-ENS & R-101 & 45.0 (+0.4) & 39.0 (+0.2) & 54.0 (+0.8) \\
            SEQ-ENS & R-101 & \textbf{46.8 (+2.2)} & \textbf{40.3 (+1.3)} & \textbf{55.1 (+1.9)} \\
        
        \Xhline{3\arrayrulewidth}
        \end{tabular}
    }
    \caption{Sequential Ensembles vs Simple Ensembles on challenging datasets.}
    \label{table:ade_coco_pascal}
\end{table}

==> tables/cityscapes.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2.7pt} %% controls col space, bigger => more space between cols
% \rowcolors{1}{}{lightgray} %%% alternating row grey color, comment to remove

\resizebox{7.0in}{!}{

    \renewcommand{\arraystretch}{1.2} % Default value: 1, controls row space
    \begin{tabular}{@{}l|l| c c c c c c c c c c c c c c c c c c c| l@{}}
    \Xhline{3\arrayrulewidth}

    \textbf{Method} & \textbf{Arch} & \textbf{road} & \textbf{swlk} & \textbf{bld.} & \textbf{wall} & \textbf{fnce} & \textbf{pole} & \textbf{tlgt} & \textbf{tsgn} & \textbf{veg} & \textbf{terain} & \textbf{sky} & \textbf{prsn} & \textbf{ridr} & \textbf{car} & \textbf{trck} & \textbf{bus} & \textbf{train} & \textbf{mcyl} & \textbf{bcyl} & \textbf{mIoU} \\
    
     \textcolor{gray}{Class (\%) $\rightarrow$} & & \textcolor{gray}{32.9} & \textcolor{gray}{4.7} & \textcolor{gray}{19.2} & \textcolor{gray}{0.6} & \textcolor{gray}{0.7} & \textcolor{gray}{1.2} & \textcolor{gray}{0.2} & \textcolor{gray}{0.6} & \textcolor{gray}{15.2} & \textcolor{gray}{0.7} & \textcolor{gray}{2.9} & \textcolor{gray}{1.1} & \textcolor{gray}{0.2} & \textcolor{gray}{5.7} & \textcolor{gray}{0.3} & \textcolor{gray}{0.3} & \textcolor{gray}{0.1} & \textcolor{gray}{0.1} & \textcolor{gray}{0.6} & \\
    
    \hline
    \footnotesize{MobileNetv3}~\cite{howard2019searching} & D8s & 95.9	& 77.6	& 87.7	& 39.4	& 47	& 52.5	& 45.1	& 63.1	& 89.8	& 54.3	& 90.2	& 71.1	& 45.1	& 90.6	& 45.7	& 64.7	& 51.5	& 39.3	& 67	& 64.1\\
    SIM-ENS & D8s & 96.1	&77.2	&88.1	&41.1	&49.1	&54.1	&48.1	&65.4	&90.2	&55.7	&91.8	&73.4	&46.4	&90.2	&47.9	&68.2	&51.5	&44.1	&68.3	&65.4 (+1.3) \\
    SEQ-ENS & D8s & \textbf{96.9}	&\textbf{79.1}	&\textbf{89.2}	&\textbf{42.6}	&\textbf{52.4}	&\textbf{56.8}	&\textbf{52.7}	&\textbf{68.3}	&\textbf{90.6}	&\textbf{58.4}	&\textbf{92.3}	&\textbf{74.5}	&\textbf{48.8}	&\textbf{91.4}	&\textbf{54.6}	&\textbf{70.8}	&\textbf{51.8}	&\textbf{47.9}	&\textbf{69.5}	&\textbf{68.7 (+4.6)}\\
    
    \hline
    \footnotesize{MobileNetv3}~\cite{howard2019searching} & D8 & 97.4	&80.9	&90.2	&48.3	&51.4	&57.1	&57.7	&69.6	&91.3	&60.1	&93.3	&75.5	&50.1	&92.7	&58.4	&73.5	&51.6	&50.3	&70.6	&69.5\\
    SIM-ENS & D8 &97.8	&81.6	&90.8	&49.0	&53.5	&58.3	&60.4	&71.6	&91.4	&61.3	&93.8	&76.4	&53.7	&93.1	&62.1	&74.5	&53.7	&54.8	&73.1	&71.1 (+1.6)\\
    SEQ-ENS & D8 &\textbf{98.1}	&\textbf{83.7}	&\textbf{91.1}	&\textbf{50.3}	&\textbf{56.8}	&\textbf{59.8}	&\textbf{65.0}	&\textbf{78.9}	&\textbf{92.0}	&\textbf{62.8}	&\textbf{94.1}	&\textbf{78.1}	&\textbf{57.8}	&\textbf{94.0}	&\textbf{68.9}	&\textbf{75.1}	&\textbf{57.4}	&\textbf{59.4}	&\textbf{75.4}	&\textbf{73.6 (+4.1)} \\
    

    \hline\hline
    HRNet~\cite{sun2019high} & H-18s &98.2	&85.5	&92.4	&53.2	&61.5	&66.4	&70.3	&77.9	&92.4	&63.8	&94.4	&81.1	&59.2	&94.4	&66.4	&84	 &70.5	&59.7	&76.1	&76.2\\
    
    SIM-ENS & H-18s &98.2	&85.6	&92.7	&56.3	&61.1	&67.1	&71.8	&79.4	&92.8	&\textbf{65.4}	&94.8	&82.4	&61.6	&94.9	&69.4	&84.4	&67.5	&61.9	&77.0	&77.1 (+0.9)\\
    
    SEQ-ENS & H-18s &\textbf{98.4}	&\textbf{86.8}	&\textbf{93.1}	&\textbf{59}	&\textbf{63.9}	&\textbf{69.2}	&\textbf{73.6}	&\textbf{79.6}	&\textbf{92.9}	&64.7	&\textbf{94.9}	&\textbf{82.8}	&\textbf{62.2}	&\textbf{95.1}	&\textbf{75.5}	&\textbf{88}	&\textbf{78}	&\textbf{63.4}	&\textbf{78.2}	&\textbf{78.9 (+2.7)}\\
    
    \hline
    HRNet~\cite{sun2019high} & H-18 &98.3	&86.4	&93.1	&59.1	&63.7	&69.3	&73.2	&80.6	&92.9	&66.4	&95	&82.8	&61.8	&94.9	&75.9	&87.7	&75.5	&60.4	&77.3	&78.7\\
    
    SIM-ENS & H-18 &98.3	&86.7	&93.3	&59.2	&63.6	&69.4	&74.1	&81.1	&93.0	&66.4	&95.3	&83.1	&62.0	&94.5	&76.5	&87.8	&74.3	&60.7	&78.1	&79.0 (+0.3)	\\
    
    SEQ-ENS & H-18 & \textbf{98.4}	&\textbf{87.1}	&\textbf{93.3}	&\textbf{58.0}	&\textbf{64.6}	&\textbf{71.0}	&\textbf{75.0}	&\textbf{82.0}	&\textbf{93.1}	&\textbf{66.4}	&\textbf{95.4}	&\textbf{84.0}	&\textbf{63.2}	&\textbf{95.2}	&\textbf{79.1}	&\textbf{90.1}	&\textbf{78.6}	&\textbf{62.7}	&\textbf{79.1}	&\textbf{79.8(+1.1)}\\
    \hline
    
    HRNet~\cite{sun2019high} & H-48 &98.5	&87.3	&93.4	&56.4	&65.6	&71.2	&75.5	&81.9	&92.9	&\textbf{63.2}	&95.3	&84.1	&66.3	&95.4	&79.7	&89.8	&84.2	&68.8	&80.1	&80.5\\
    
    SIM-ENS & H-48 & 98.6	&87.1	&93.4	&56.6	&65.1	&71.6	&75.8	&82.1	&92.9	&63.1	&95.4	&84.2	&67.1	&95.6	&79.8	&89.9	&84.6	&68.3	&79.9	&80.6 (+0.1)\\
    
    SEQ-ENS & H-48 & \textbf{98.6}	&\textbf{88.0}	&\textbf{93.7}	&\textbf{58.9}	&\textbf{66.9}	&\textbf{72.6}	&\textbf{76.8}	&\textbf{83.2}	&\textbf{93.1}	&62.9	&\textbf{95.7}	&\textbf{84.8}	&\textbf{68.3}	&\textbf{95.7}	&\textbf{80.1}	&\textbf{90.6}	&\textbf{85.6}	&\textbf{68.8}	&\textbf{80.9}	&\textbf{81.3 (+0.8)}\\
    
    \hline\hline
    DeepLabv3+~\cite{chen2018encoder} & R-18 & 98.0	&84.4	&92.3	&51.4	&58.2	&66.1	&69.9	&77.6	&92.2	&63.6	&94.4	&81.3	&60.8	&94.7	&76.1	&85.4	&72.5	&63.1	&76.3	&76.8 \\
    SIM-ENS & R-18 & 98.1	&85.0	&92.6	&51.1	&58.3	&67.3	&71.5	&78.9	&92.4	&64.1	&94.7	&82.1	&61.0	&95.0	&77.8	&87.3	&74.5	&64.3	&76.9	&77.8 (+1.0)\\
    SEQ-ENS & R-18 & \textbf{98.3}	&\textbf{86.3}	&\textbf{93.1}	&\textbf{51.2}	&\textbf{59.4}	&\textbf{69.8}	&\textbf{74.6}	&\textbf{80.8}	&\textbf{92.7}	&\textbf{64.9}	&\textbf{95.0}	&\textbf{83.6}	&\textbf{62.8}	&\textbf{95.6}	&\textbf{79.8}	&\textbf{88.1}	&\textbf{77.0}	&\textbf{67.2}	&\textbf{78.3}	&\textbf{78.9 (+2.1)}\\
    
    \hline
    DeepLabv3+~\cite{chen2018encoder} & R-50 &98.4	&86.6	&93	&51.2	&62.5	&69.5	&74.3	&82.2	&92.7	&63.5	&94.9	&84.2	&65.8	&95.6	&81.1	&88.8	&84.7	&68.6	&79.5	&79.8\\
    SIM-ENS & R-50 &98.5	&86.8	&93.1	&51.8	&62.8	&70.1	&74.5	&82.8	&92.7	&63.7	&95.0	&84.6	&65.9	&95.4	&\textbf{81.4}	&89.8	&85.1	&69.2	&79.8	&80.1 (+0.3)\\
    SEQ-ENS & R-50 & \textbf{98.5}	&\textbf{87.3}	&\textbf{93.3}	&\textbf{53.4}	&\textbf{63.2}	&\textbf{71.2}	&\textbf{75.6}	&\textbf{83.5}	&\textbf{92.9}	&\textbf{65.4}	&\textbf{95.2}	&\textbf{85.0}	&\textbf{66.3}	&\textbf{95.8}	&79.3	&\textbf{91.9}	&\textbf{85.2}	&\textbf{70.0}	&\textbf{80.2}	&\textbf{80.7 (+0.9)} \\
    
    \hline
    DeepLabv3+~\cite{chen2018encoder} & R-101 &98.4	&86.4	&93.4	&54.9	&64.4	&70.2	&74.6	&81.9	&93.0	&62.4	&95.1	&84.6	&67.7	&95.8	&85.2	&91.8	&85.2	&71.3	&80.3	&80.9 \\
    SIM-ENS & R-101 & 98.4	&86.7	&93.4	&55.1	&64.6	&70.1	&74.7	&82.0	&92.8	&62.8	&95.4	&84.7	&67.8	&\textbf{96.3}	&85.0	&91.9	&85.8	&71.9	&80.3	&81.1 (+0.2) \\
    SEQ-ENS & R-101 &\textbf{98.5}	&\textbf{87.0}	&\textbf{93.5}	&\textbf{56.0}	&\textbf{64.6}	&\textbf{71.1}	&\textbf{75.2}	&\textbf{82.6}	&\textbf{93.1}	&\textbf{63.5}	&\textbf{95.4}	&\textbf{84.9}	&\textbf{68.5}	&96.0	&\textbf{85.4}	&\textbf{92.3}	&\textbf{86.5}	&\textbf{72.5}	&\textbf{80.5}	&\textbf{81.5 (+0.6)} \\
    
    
    \Xhline{3\arrayrulewidth}
    
    \end{tabular}
}
    
\caption{Comparison of Sequential Ensembles (Ours) with Simple Ensembles for $N=2$ on the Cityscapes \texttt{val} set. R-@ and H-@ stand for ResNet-@ and HRNet-W@ respectively. D8 is the output stride of DeepLabv3+. \texttt{s} denotes the \textit{small} version of the backbone. Without using any extra data, all models are trained at the image resolution of $512 \times 1024$ and tested at $1024 \times 2048$ using single-scale inference. }
\label{table:cityscapes}

\end{table*}

==> tables/cityscapes_backbone_trend.tex <==
\begin{table}[b]
\centering
\small
\resizebox{1.7in}{!}{
        \renewcommand{\arraystretch}{1.2}
        \rowcolors{1}{}{lightgray}
        \setlength{\tabcolsep}{3pt}
        \begin{tabular}{@{}l| c  c  c c@{}}
            \Xhline{3\arrayrulewidth}
            \diagbox{$\mathbf{G_0}$}{$\mathbf{G_1}$}   & -   & \textbf{H-18s}   & \textbf{H-18} & \textbf{H-48}   \\
            \hline
            \textbf{H-18s}   &   76.2    &   78.9    &   79.3    &   80.3   \\
            \textbf{H-18}    &   78.7    &   79.8    &   79.8    &   81.0   \\
            \textbf{H-48}    &   80.5    &   80.7    &   80.9    &   81.3   \\
            \Xhline{3\arrayrulewidth}
        \end{tabular}
        }
\thinspace
\resizebox{1.5in}{!}{
        \renewcommand{\arraystretch}{1.2}
        \rowcolors{1}{}{lightgray}
        \setlength{\tabcolsep}{3pt}
        \begin{tabular}{@{}l| c c c@{}}
            \Xhline{3\arrayrulewidth}
            \textbf{Arch}   & $\mathbf{G_0}$   & $\mathbf{G_i}$   & $\Delta \mathbf{G}$  \\
            \hline
            \textbf{H-18s}  &  3.9M    &   4.5M & +15.4\%  \\
            \textbf{H-18}   &  9.6M    &   10.5M & +9.3\%\\
            \textbf{H-48}   &  65.8M   &   69.4M & +5.5 \%  \\
            \Xhline{3\arrayrulewidth}
        \end{tabular}
        }
    \caption{\textit{Left}: Sequential ensembles (mIoU) gains with various backbone combinations of HRNet~\cite{sun2019high} on the Cityscapes \texttt{val} set. \textit{Right}: Number of parameters when using \textit{ten} ADON blocks in $G_i$.}
    
\label{table:cityscapes_backbone_trend}
\end{table}


==> tables/prev_sim_ens_compare.tex <==
\begin{table*}[t]
\centering
\small
% \setlength{\tabcolsep}{2.7pt} %% controls col space, bigger => more space between cols
% \rowcolors{1}{}{lightgray} %%% alternating row grey color, comment to remove
\setlength{\belowcaptionskip}{-10pt}
\resizebox{7.0in}{!}{

    \renewcommand{\arraystretch}{1.2} % Default value: 1, controls row space
    \begin{tabular}{@{}l|l| c c c c c c c c c c c c c c| l |l| l| l@{}}
    \Xhline{3\arrayrulewidth}

    \multirow{2}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{Arch}} & \multicolumn{15}{c|}{\textbf{Cityscapes (val)}} &  \multirow{3}{*}{\textbf{ADE-20K}}  & \multirow{3}{*}{\textbf{COCO-Stuff}} & \multirow{3}{*}{\footnotesize{\textbf{PASCAL-Context}}}\\
    
    % \cmidrule(lr){3-17}
    
    & & \textbf{wall} & \textbf{fnce} & \textbf{pole} & \textbf{tlgt} & \textbf{tsgn} & \textbf{terain} & \textbf{sky} & \textbf{prsn} & \textbf{ridr} &  \textbf{trck} & \textbf{bus} & \textbf{train} & \textbf{mcyl} & \textbf{bcyl} & \textbf{mIoU} & & &\\
    
     \textcolor{gray}{Class (\%) $\rightarrow$} & & \textcolor{gray}{0.6} & \textcolor{gray}{0.7} & \textcolor{gray}{1.2} & \textcolor{gray}{0.2} & \textcolor{gray}{0.6} & \textcolor{gray}{0.7} & \textcolor{gray}{2.9} & \textcolor{gray}{1.1} & \textcolor{gray}{0.2} &  \textcolor{gray}{0.3} & \textcolor{gray}{0.3} & \textcolor{gray}{0.1} & \textcolor{gray}{0.1} & \textcolor{gray}{0.6} & & (val) & (test) & (test)\\

    \hline
    \footnotesize{MobileNetv3}~\cite{howard2019searching} & D8s & 39.4	& 47	& 52.5	& 45.1	& 63.1	& 54.3	& 90.2	& 71.1	& 45.1	& 45.7	& 64.7	& 51.5	& 39.3	& 67	& 64.1 & 29.7 & 24.1 & 32.7\\
    
    SIM-ENS & D8s 	&41.1	&49.1	&54.1	&48.1	&65.4	&55.7	&91.8	&73.4	&46.4	&47.9	&68.2	&51.5	&44.1	&68.3	&65.4 (+1.3) & 31.4 (+1.7) & 26.3 (+2.2) & 34.2 (+1.5)\\
    
    SEQ-ENS & D8s 	&\textbf{42.6}	&\textbf{52.4}	&\textbf{56.8}	&\textbf{52.7}	&\textbf{68.3}	&\textbf{58.4}	&\textbf{92.3}	&\textbf{74.5}	&\textbf{48.8}	&\textbf{54.6}	&\textbf{70.8}	&\textbf{51.8}	&\textbf{47.9}	&\textbf{69.5}	&\textbf{68.7 (+4.6)} & \textbf{35.3 (+5.6)} & \textbf{28.6 (+4.5)}  & \textbf{36.9 (+4.2)}\\
    
    \hline
    \footnotesize{MobileNetv3}~\cite{howard2019searching} & D8 	&48.3	&51.4	&57.1	&57.7	&69.6		&60.1	&93.3	&75.5	&50.1	&58.4	&73.5	&51.6	&50.3	&70.6	&69.5 & 31.8 & 26.8 & 34.4\\
    
    SIM-ENS & D8 	&49.0	&53.5	&58.3	&60.4	&71.6	&61.3	&93.8	&76.4	&53.7	&62.1	&74.5	&53.7	&54.8	&73.1	&71.1 (+1.6) & 33.9 (+2.1) & 28.5 (+1.7) & 36.0 (+1.6)\\
    
    SEQ-ENS & D8 	&\textbf{50.3}	&\textbf{56.8}	&\textbf{59.8}	&\textbf{65.0}	&\textbf{78.9}	&\textbf{62.8}	&\textbf{94.1}	&\textbf{78.1}	&\textbf{57.8}	&\textbf{68.9}	&\textbf{75.1}	&\textbf{57.4}	&\textbf{59.4}	&\textbf{75.4}	&\textbf{73.6 (+4.1)} & \textbf{35.6 (+3.8)} & \textbf{30.0 (+3.2)} & \textbf{37.3 (+2.9)}\\
    

    \hline\hline
    HRNet~\cite{sun2019high} & H-18s 	&53.2	&61.5	&66.4	&70.3	&77.9	&63.8	&94.4	&81.1	&59.2	&66.4	&84	 &70.5	&59.7	&76.1	&76.2 & 33.1 & 29.4 & 38.9 \\
    
    SIM-ENS & H-18s 	&56.3	&61.1	&67.1	&71.8	&79.4	&\textbf{65.4}	&94.8	&82.4	&61.6		&69.4	&84.4	&67.5	&61.9	&77.0	&77.1 (+0.9) & 34.5 (+1.4) & 30.0 (+0.6) & 40.4 (+1.5) \\
    
    SEQ-ENS & H-18s 	&\textbf{59}	&\textbf{63.9}	&\textbf{69.2}	&\textbf{73.6}	&\textbf{79.6}	&64.7	&\textbf{94.9}	&\textbf{82.8}	&\textbf{62.2}	&\textbf{75.5}	&\textbf{88}	&\textbf{78}	&\textbf{63.4}	&\textbf{78.2}	&\textbf{78.9 (+2.7)} & \textbf{37.6 (+4.5)} & \textbf{32.7 (+3.3)} & \textbf{42.0 (+3.1)}\\
    
    \hline
    HRNet~\cite{sun2019high} & H-18 	&59.1	&63.7	&69.3	&73.2	&80.6	&66.4	&95	&82.8	&61.8	&75.9	&87.7	&75.5	&60.4	&77.3	&78.7 & 36.8 & 33.0 & 42.6\\
    
    SIM-ENS & H-18 	&59.2	&63.6	&69.4	&74.1	&81.1	&66.4	&95.3	&83.1	&62.0	&76.5	&87.8	&74.3	&60.7	&78.1	&79.0 (+0.3) & 37.6 (+0.8) & 34.1 (+1.1) & 43.9 (+1.3)	\\
    
    SEQ-ENS & H-18 	&\textbf{58.0}	&\textbf{64.6}	&\textbf{71.0}	&\textbf{75.0}	&\textbf{82.0}	&\textbf{66.4}	&\textbf{95.4}	&\textbf{84.0}	&\textbf{63.2}	&\textbf{79.1}	&\textbf{90.1}	&\textbf{78.6}	&\textbf{62.7}	&\textbf{79.1}	&\textbf{79.8(+1.1)} & \textbf{40.9 (+4.1)} & \textbf{35.7 (+2.7)} & \textbf{46.1 (+3.5)}\\
    \hline
    
    HRNet~\cite{sun2019high} & H-48 	&56.4	&65.6	&71.2	&75.5	&81.9	&\textbf{63.2}	&95.3	&84.1	&66.3	&79.7	&89.8	&84.2	&68.8	&80.1	&80.5 & 42.0 & 38.3 & 51.1\\
    
    SIM-ENS & H-48 	&56.6	&65.1	&71.6	&75.8	&82.1	&63.1	&95.4	&84.2	&67.1	&79.8	&89.9	&84.6	&68.3	&79.9	&80.6 (+0.1) & 42.5 (+0.5) & 39.7 (+1.4) & 52.1 (+1.0)\\
    
    SEQ-ENS & H-48 	&\textbf{58.9}	&\textbf{66.9}	&\textbf{72.6}	&\textbf{76.8}	&\textbf{83.2}	&62.9	&\textbf{95.7}	&\textbf{84.8}	&\textbf{68.3}	&\textbf{80.1}	&\textbf{90.6}	&\textbf{85.6}	&\textbf{68.8}	&\textbf{80.9}	&\textbf{81.3 (+0.8)} & \textbf{45.6 (+3.6)} & \textbf{40.8 (+2.5)} & \textbf{53.8 (+2.7)}\\
    
    \hline\hline
    DeepLabv3+~\cite{chen2018encoder} & R-18 	&51.4	&58.2	&66.1	&69.9	&77.6	&63.6	&94.4	&81.3	&60.8	&76.1	&85.4	&72.5	&63.1	&76.3	&76.8 & 34.1 & 29.7 & 43.5\\
    
    SIM-ENS & R-18	&51.1	&58.3	&67.3	&71.5	&78.9	&64.1	&94.7	&82.1	&61.0	&77.8	&87.3	&74.5	&64.3	&76.9	&77.8 (+1.0) & 35.4 (+1.3) & 31.2 (+1.5) & 45.8 (+2.3)\\
    
    SEQ-ENS & R-18 	&\textbf{51.2}	&\textbf{59.4}	&\textbf{69.8}	&\textbf{74.6}	&\textbf{80.8}	&\textbf{64.9}	&\textbf{95.0}	&\textbf{83.6}	&\textbf{62.8}	&\textbf{79.8}	&\textbf{88.1}	&\textbf{77.0}	&\textbf{67.2}	&\textbf{78.3}	&\textbf{78.9 (+2.1)} & \textbf{37.6 (+3.5)} & \textbf{35.3 (+4.1)} & \textbf{46.2 (+2.7)}\\
    
    \hline
    DeepLabv3+~\cite{chen2018encoder} & R-50 	&51.2	&62.5	&69.5	&74.3	&82.2	&63.5	&94.9	&84.2	&65.8	&81.1	&88.8	&84.7	&68.6	&79.5	&79.8 & 42.7 & 37.4 & 50.4\\
    
    SIM-ENS & R-50 	&51.8	&62.8	&70.1	&74.5	&82.8	&63.7	&95.0	&84.6	&65.9		&\textbf{81.4}	&89.8	&85.1	&69.2	&79.8	&80.1 (+0.3) & 43.3 (+0.6) & 38.2 (+0.8) & 51.8 (+1.4)\\
    
    SEQ-ENS & R-50  &\textbf{53.4}	&\textbf{63.2}	&\textbf{71.2}	&\textbf{75.6}	&\textbf{83.5}	&\textbf{65.4}	&\textbf{95.2}	&\textbf{85.0}	&\textbf{66.3}		&79.3	&\textbf{91.9}	&\textbf{85.2}	&\textbf{70.0}	&\textbf{80.2}	&\textbf{80.7 (+0.9)} & \textbf{45.1 (+2.4)} & \textbf{39.2 (+1.8)} &  \textbf{52.4 (+2.0)}\\
    
    \hline
    DeepLabv3+~\cite{chen2018encoder} & R-101 	&54.9	&64.4	&70.2	&74.6	&81.9	&62.4	&95.1	&84.6	&67.7	&85.2	&91.8	&85.2	&71.3	&80.3	&80.9  & 44.6 & 38.8 & 53.2\\
    
    SIM-ENS & R-101 	&55.1	&64.6	&70.1	&74.7	&82.0	&62.8	&95.4	&84.7	&67.8	&85.0	&91.9	&85.8	&71.9	&80.3	&81.1 (+0.2) & 45.0 (+0.4) & 39.0 (+0.2) & 54.0 (+0.8)\\
    
    SEQ-ENS & R-101 	&\textbf{56.0}	&\textbf{64.6}	&\textbf{71.1}	&\textbf{75.2}	&\textbf{82.6}	&\textbf{63.5}	&\textbf{95.4}	&\textbf{84.9}	&\textbf{68.5}	&\textbf{85.4}	&\textbf{92.3}	&\textbf{86.5}	&\textbf{72.5}	&\textbf{80.5}	&\textbf{81.5 (+0.6)} & \textbf{46.8 (+2.2)} & \textbf{40.3 (+1.3)} & \textbf{55.1 (+1.9)}\\
    
    
    \Xhline{3\arrayrulewidth}
    
    \end{tabular}
}
    
\caption{Comparison of Sequential Ensembles (Ours) with Simple Ensembles using $N=2$ on various datasets. R-@ and H-@ stand for ResNet-@ and HRNet-W@ respectively. D8 is the output stride of DeepLabv3+. \texttt{s} denotes the \textit{small} version of the backbone. We report class-wise mIoU for 15 rare classes (except road, building, vegetation, car, sidewalk) in Cityscapes. For rare classes such as \textit{mcyl}, SEQ-ENS improves mIOU by $\approx 2X$ compared to SIM-ENS.}
\label{table:sim_ens_compare}
\vspace*{-0.1in}
\end{table*}
